Magnetic Sensor Compensation Utilizing Factor Graph Estimation

Recently, there has been significant interest in the ability to navigate without GPS using the magnetic anomaly field of the Earth (magnav). One of the key technical bottlenecks to achieving magnav is obtaining an accurate magnetic sensor calibration, taking into account own-ship and sensor effects. The Tolles-Lawson magnetic calibration method was developed when airborne magnetic survey aircraft were first employed 80 years ago. In this paper, we present a magnetic calibration algorithm based on a factor graph optimization using inertial measurements as well as inputs from both a vector and scalar magnetometer. The factor graph is well suited for combining multiple sensor inputs and allows accurate calibrations in the presence of large permanent moments as well as estimating a time-varying external magnetic field during the calibration, two problems that are difficult to solve with previous approaches. The ability to accurately calibrate a magnetic sensor in flight (i.e. with the presence of a large platform field and a varying Earth field due to movement) will allow greater flexibility in sensor mounting locations for magnetic anomaly navigation.

==> 4_support/figures.tex <==
% A common file to store all figure definitions
%
% In preparing your thesis, one of the first things you should do is
% organize your figures.  Then, one of the last things you'll do is
% reorder your figures so they display where you want them to in the
% text.  Organizing figure definitions in a common files helps:
%
%   1. Write new figures using earlier examples.
%
%   2.  Isolate code and minimize the risk of introducing bugs in the
%   final editing process.  Trust me, moving around just one line of
%   code is easier.
%
%   3.  Reuse figures in other papers.  <=== the best reason!
%
% Note command names can not include numbers and special characters.
%
% To make the file more searchable, use naming conventions that map
% the graphics filename labSetup.jpg to the command name \figlabSetup to the
% figure label fig:labSetup.
% 

\newcommand{\fignonorthodiagram}{\begin{figure}[htbp]
  \centering

        \begin{tikzpicture}
               [tdplot_main_coords, 
               axis/.style={->,blue,thick},
               vector/.style={-stealth,black,very thick},
               vector guide/.style={dashed,red,thick},
               angle/.style={<->,red}]
          
          \coordinate (O) at (0,0,0);
          \begin{scope}[local bounding box=L]
          % axes
          \draw[axis] (0,0,-1.5) -- ( 0,0,3.5) node[anchor=south east]{$z$};
          \draw[axis] (0,-1,-.5) -- ( 0,4,-.5) node[anchor=west]{$y$};
         
          \draw[axis] (-1,0,-.5) -- ( 4,0,-.5) node[anchor=south west]{$x$};
        
          % vector 1
          \def\az{-.5}
          \def\ay{0}
          \def\ax{3}
        
          \draw[vector] (0,0,-.5) -- (\ax,\ay,\az) node[anchor=south]{$m_x$};
            
          %  % vector 2
          \def\bz{-1.5}
          \def\by{3}
          \def\bx{2}
          \draw[vector] (0,0,-.5) -- (\bx,\by,\bz) node[anchor=west]{$m_y$};
        
          %  % vector 3 
          \def\cz{2.5}
          \def\cy{0}
          \def\cx{.5}
          \draw[vector] (0,0,-.5) -- (\cx,\cy,\cz) node[anchor=north]{$m_z$};
        
           % dashed lines
          %  % m_y
          \draw[dashed,gray] (\bx,\by,\bz) -- (\bx,\by,-.5);
          \draw[dashed,gray] (\bx,\by,-.5) -- (\bx,0,-.5);
          \draw[dashed,gray] (\bx,\by,-.5) -- (0,\by,-.5);
          \draw[dashed,gray] (\bx,\by,-.5) -- (0,0,-.5);
          
        
            
          % arcs
        
          \tdplotdefinepoints(0,0,-.5)(\bx,\by,-1.5)(\bx,\by,-.5)
          \tdplotdrawpolytopearc[angle]{2.5}{anchor=east}{$\gamma$}
        
          \tdplotdefinepoints(0,0,-.5)(2,3,-.5)(0,1,-.5)
          \tdplotdrawpolytopearc[angle]{2.75}{anchor=east}{$\beta$}
        
          \tdplotdefinepoints(0,0,-.5)(0,0,3.5)(.5,0,2.5)
          \tdplotdrawpolytopearc[angle]{2.5}{anchor=south}{$\alpha$}
          \end{scope}

          \begin{scope}
            \hspace*{-1.2cm}
            \includegraphics[scale=.3, keepaspectratio]{5_figures/plane_profile.png}
          \end{scope}
        
        \end{tikzpicture}
        \caption{Non-Orthogonal Measurements in Sensor Frame}
        \label{fig:non_ortho}
\end{figure}
}

\newcommand{\figSensorPics}{\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{.49\textwidth}
        \includegraphics[width=\textwidth, keepaspectratio]{Pictures/MFAM.png}
        \caption{Geometrics MFAM \citep{website:MFAM}}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.49\textwidth}
        \includegraphics[width=\textwidth, keepaspectratio]{Pictures/VMR.png}
        \caption{TwinLeaf VMR \citep{website:VMR}}
    \end{subfigure}    
    \caption{}
    \label{fig:my_label}
\end{figure}
 }

\newcommand{\figVMRTempEffect}{\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{.49\textwidth}
        \includegraphics[width=\textwidth, keepaspectratio]{5_figures/VMR Temperature Plot.png}
        \caption{Temperature Effects on VMR}
        \label{fig:VMR T}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.49\textwidth}
        \includegraphics[width=\textwidth, keepaspectratio]{5_figures/MFAM_VMR_Mag_uncomp.png}
        \caption{VMR and MFAM Measurements}
        \label{fig:VMR_temp_uncomp}  
    \end{subfigure}
    \caption{VMR Temperature Effects}
    \label{fig:VMR_Temp_EF}
\end{figure}
}


\newcommand{\figFactorGraph}{\begin{figure}[H]
    \centering
    \begin{tikzpicture}[
    roundnode/.style={circle, draw=black!100, very thick, minimum size=10mm},
    squarednode/.style={rectangle, draw=black!100, fill=black!100, very thick, text=white},
    dotnode/.style={rectangle, draw=white!100},
    gyronode/.style={rectangle, draw=black!100, fill=black!50},
    dynanode/.style={rectangle, draw=black!100, fill=green!50}
    ]
    %Nodes
    
    \node[roundnode]        (C0)    at (0,2)  {$\bm{C}_{n}^{b0}$};
    \node[roundnode]        (C1)    at (3,2)  {$\bm{C}_{n}^{b1}$};
    \node[roundnode]        (C2)    at (6,2) {$\bm{C}_{n}^{b2}$};
    \node[roundnode]        (C3)    at (9,2) {$\bm{C}_{n}^{b3}$};

    \node[squarednode]      (m0)    at (0,0) {$m^{b0}$};
    \node[squarednode]      (m1)    at (3,0) {$m^{b1}$};
    \node[squarednode]      (m2)    at (6,0) {$m^{b2}$};
    \node[squarednode]      (m3)    at (9,0) {$m^{b3}$};

    \node[gyronode]       (rpy0)  at  (0,4) {$\bm{rpy}^{b0}$};
    \node[gyronode]       (rpy1)  at  (3,4) {$\bm{rpy}^{b1}$};
    \node[gyronode]       (rpy2)  at  (6,4) {$\bm{rpy}^{b2}$};
    \node[gyronode]       (rpy3)  at  (9,4) {$\bm{rpy}^{b3}$};
    
    \node[roundnode]        (b)     at (-2,1.5) {$\bm{h}_{hi}$};
    
    \node[dynanode]         (d1)    at (1.5,-4) {$\bm{d}^1$};
    \node[dynanode]         (d2)    at (4.5,-4) {$\bm{d}^2$};
    \node[dynanode]         (d3)    at (7.5,-4) {$\bm{d}^3$};

    \node[roundnode]        (e0)    at (0,-4) {$\bm{e}^{n0}$};
    \node[roundnode]        (e1)    at (3,-4) {$\bm{e}^{n1}$};
    \node[roundnode]        (e2)    at (6,-4) {$\bm{e}^{n2}$};
    \node[roundnode]        (e3)    at (9,-4) {$\bm{e}^{n3}$};
    
    \node[dotnode]        (Cdots)   at (10.5,2) {\dots};
    \node[dotnode]        (mdots)   at (10.5,0) {\dots};
    \node[dotnode]        (mdots)   at (10.5,-2) {\dots};

    \node[gyronode]        (omega1)     at (1.5,2) {$\bm{\omega}^1$};
    \node[gyronode]        (omega2)     at (4.5,2) {$\bm{\omega}^2$};
    \node[gyronode]        (omega3)     at (7.5,2) {$\bm{\omega}^3$};

    \node[roundnode]        (T)     at (-2,-3.5) {$\bm{T}$};
    \node[roundnode]        (bias)     at (-3,-2) {$\bm{h}_{vec}$};

    %Lines
    \draw[-] (e0) -- (d1);
    \draw[-] (d1) -- (e1);
    \draw[-] (e1) -- (d2);
    \draw[-] (d2) -- (e2);
    \draw[-] (e2) -- (d3);
    \draw[-] (d3) -- (e3);
    \draw[-] (e0) -- (m0);
    \draw[-] (e1) -- (m1);
    \draw[-] (e2) -- (m2);
    \draw[-] (e3) -- (m3);
    \draw[-] (b) -- (m0);
    \draw[-] (b) -- (m1);
    \draw[-] (b) -- (m2);
    \draw[-] (b) -- (m3);
    \draw[-] (C0) -- (m0);
    \draw[-] (C1) -- (m1);
    \draw[-] (C2) -- (m2);
    \draw[-] (C3) -- (m3);
    \draw[-] (C0) -- (rpy0);
    \draw[-] (C1) -- (rpy1);
    \draw[-] (C2) -- (rpy2);
    \draw[-] (C3) -- (rpy3);
    \draw[-] (C0) -- (omega1);
    \draw[-] (C1) -- (omega1);
    \draw[-] (C1) -- (omega2);
    \draw[-] (C2) -- (omega2);
    \draw[-] (C2) -- (omega3);
    \draw[-] (C3) -- (omega3);

    \draw[-] (T) -- (m0);
    \draw[-] (T) -- (m1);
    \draw[-] (T) -- (m2);
    \draw[-] (T) -- (m3);
    
    \draw[-] (bias) -- (m0);
    \draw[-] (bias) -- (m1);
    \draw[-] (bias) -- (m2);
    \draw[-] (bias) -- (m3);

    \end{tikzpicture}
    \caption{Time Variant Magnetic Calibration Factor Graph}
    \label{fig:FG}
\end{figure}
}

\newcommand{\figFactorGraphConstant}{\begin{figure}[htbp]
    \centering
    \begin{tikzpicture}[
    roundnode/.style={circle, draw=black!100, very thick, minimum size=10mm},
    squarednode/.style={rectangle, draw=black!100, fill=black!100, very thick, text=white},
    dotnode/.style={rectangle, draw=white!100},
    gyronode/.style={rectangle, draw=black!100, fill=black!50},
    dynanode/.style={rectangle, draw=black!100, fill=green!50}
    ]
    %Nodes
    
    \node[roundnode]        (C0)    at (0,2)  {$\bm{C}_{n}^{b0}$};
    \node[roundnode]        (C1)    at (3,2)  {$\bm{C}_{n}^{b1}$};
    \node[roundnode]        (C2)    at (6,2) {$\bm{C}_{n}^{b2}$};
    \node[roundnode]        (C3)    at (9,2) {$\bm{C}_{n}^{b3}$};

    \node[squarednode]      (m0)    at (0,0) {$m^{b0}$};
    \node[squarednode]      (m1)    at (3,0) {$m^{b1}$};
    \node[squarednode]      (m2)    at (6,0) {$m^{b2}$};
    \node[squarednode]      (m3)    at (9,0) {$m^{b3}$};

    \node[gyronode]       (rpy0)  at  (0,4) {$\bm{rpy}^{b0}$};
    \node[gyronode]       (rpy1)  at  (3,4) {$\bm{rpy}^{b1}$};
    \node[gyronode]       (rpy2)  at  (6,4) {$\bm{rpy}^{b2}$};
    \node[gyronode]       (rpy3)  at  (9,4) {$\bm{rpy}^{b3}$};
    
    \node[roundnode]        (b)     at (-2,1.5) {$\bm{h}_{hi}$};

    \node[roundnode]        (e)    at (4.5,-4) {$\bm{e}^{n}$};
    
    \node[dotnode]        (Cdots)   at (10.5,2) {\dots};
    \node[dotnode]        (mdots)   at (10.5,0) {\dots};
    \node[dotnode]        (mdots)   at (10.5,-2) {\dots};

    \node[gyronode]        (omega1)     at (1.5,2) {$\bm{\omega}^1$};
    \node[gyronode]        (omega2)     at (4.5,2) {$\bm{\omega}^2$};
    \node[gyronode]        (omega3)     at (7.5,2) {$\bm{\omega}^3$};

    \node[roundnode]        (T)     at (-2,-3.5) {$\bm{T}$};
    \node[roundnode]        (bias)     at (-3,-2) {$\bm{h}_{vec}$};

    %Lines
   
    \draw[-] (e) -- (m0);
    \draw[-] (e) -- (m1);
    \draw[-] (e) -- (m2);
    \draw[-] (e) -- (m3);
    \draw[-] (b) -- (m0);
    \draw[-] (b) -- (m1);
    \draw[-] (b) -- (m2);
    \draw[-] (b) -- (m3);
    \draw[-] (C0) -- (m0);
    \draw[-] (C1) -- (m1);
    \draw[-] (C2) -- (m2);
    \draw[-] (C3) -- (m3);
    \draw[-] (C0) -- (rpy0);
    \draw[-] (C1) -- (rpy1);
    \draw[-] (C2) -- (rpy2);
    \draw[-] (C3) -- (rpy3);
    \draw[-] (C0) -- (omega1);
    \draw[-] (C1) -- (omega1);
    \draw[-] (C1) -- (omega2);
    \draw[-] (C2) -- (omega2);
    \draw[-] (C2) -- (omega3);
    \draw[-] (C3) -- (omega3);

    \draw[-] (T) -- (m0);
    \draw[-] (T) -- (m1);
    \draw[-] (T) -- (m2);
    \draw[-] (T) -- (m3);
    
    \draw[-] (bias) -- (m0);
    \draw[-] (bias) -- (m1);
    \draw[-] (bias) -- (m2);
    \draw[-] (bias) -- (m3);

    \end{tikzpicture}
    \caption{Time Invariant Magnetic Calibration Factor Graph}
    \label{fig:FG_Invariant}
\end{figure}
}

\newcommand{\figVMRComp}{\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{.49\textwidth}
        \includegraphics[width=\textwidth]{5_figures/MFAM_VMR_Mag_comp.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.49\textwidth}
        \includegraphics[width=\textwidth]{5_figures/MFAM_VMR_Mag_comp_zoom.png}
    \end{subfigure}
    \caption{Temperature Compensated VMR Measurements}
    \label{fig:VMR_Temp_Comp}
\end{figure}
}

\newcommand{\figTestSetup}{\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{.45\textwidth}
        \includegraphics[width=\textwidth, keepaspectratio]{Pictures/tripod_anotated.png}
        \caption{Test Platform}
        \label{fig:Tripod}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.45\textwidth}
    \includegraphics[trim = {70 30 70 70}, clip,width=\textwidth]{5_figures/cal_profile.png}
     \caption{Calibration profile}
     \label{fig:cal_profile}
    \end{subfigure}
    \caption{Evaluation Setup}
    \label{fig:Test_Setup}
\end{figure}
}

\newcommand{\figboxplot}{\begin{figure}[htbp]
 \begin{center}
    \includegraphics[width=5in]{5_figures/BoxPlot.png}
     \caption{Factor Graph Error Metrics}
     \label{fig:box_plot}{Note: $\epsilon_{scale}$ is unitless, while $\epsilon_{orth}$ is radians}
 \end{center}
\end{figure}
}


\newcommand{\figavgest}{\begin{figure}[htbp]
 \begin{center}
    \includegraphics[trim = {10 8 40 20}, clip,width=.5\textwidth]{5_figures/RMSE_012.png}
     \caption{External Field Magnitude Estimate}
     \label{fig:e_est}
 \end{center}
\end{figure}
}

\newcommand{\figMagDelta}{\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{.3\textwidth}
        \includegraphics[width=\textwidth]{5_figures/delta_x.png}
    \end{subfigure}
    \begin{subfigure}[b]{.3\textwidth}
        \includegraphics[width=\textwidth]{5_figures/delta_y.png}
    \end{subfigure}
    \begin{subfigure}[b]{.3\textwidth}
        \includegraphics[width=\textwidth]{5_figures/delta_z.png}
    \end{subfigure}
    \caption{Adding Permanent Magnet}
    \label{fig:MagDelta}
\end{figure}
}

\newcommand{\figBoxPlotComparison}{\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{.35\textwidth}
        \includegraphics[height=\textwidth]{5_figures/BoxPlot10.png}
        \caption{$\|\bf{e}^{n}\|$ with $10 nT/\sqrt{hr}$ Random Walk}
        \label{fig:box_plot_varying10}
    \end{subfigure}
    \begin{subfigure}[b]{.35\textwidth}
        \includegraphics[height=\textwidth]{5_figures/BoxPlot20.png}
        \caption{$\|\bf{e}^{n}\|$ with $15 nT/\sqrt{hr}$ Random Walk}
        \label{fig:box_plot_varying20}
    \end{subfigure}
    \caption{Estimation Performance in a Changing External Field}
    \label{fig:box_plot_comparison}
\end{figure}
}

\newcommand{\figBoxPlotHardIron}{\begin{figure}[htbp]
    \begin{center}
        \includegraphics[width=\textwidth]{5_figures/h_hi_variation.png}
        \caption{Hard Iron Magnitude Effect on Estimation Accuracy}
        \label{fig:h_hi_variation}
    \end{center}
\end{figure}
}

\newcommand{\figboxplotvecbias}{\begin{figure}[htbp]
    \begin{center}
        \includegraphics[width=\textwidth]{5_figures/h_vec_variation.png}
        \caption{Vector Magnetometer Bias Effect}
        \label{fig:h_vec_variation}
    \end{center}
\end{figure}
}
